A Measurement Study of TCP Performance for Chunk Delivery in DASH

Dynamic Adaptive Streaming over HTTP (DASH) has emerged as an increasingly popular paradigm for video streaming [13], in which a video is segmented into many chunks delivered to users by HTTP request/response over Transmission Control Protocol (TCP) con- nections. Therefore, it is intriguing to study the performance of strategies implemented in conventional TCPs, which are not dedicated for video streaming, e.g., whether chunks are efficiently delivered when users per- form interactions with the video players. In this paper, we conduct mea- surement studies on users chunk requesting traces in DASH from a rep- resentative video streaming provider, to investigate users behaviors in DASH, and TCP-connection-level traces from CDN servers, to investi- gate the performance of TCP for DASH. By studying how video chunks are delivered in both the slow start and congestion avoidance phases, our observations have revealed the performance characteristics of TCP for DASH as follows: (1) Request patterns in DASH have a great impact on the performance of TCP variations including cubic; (2) Strategies in conventional TCPs may cause user perceived quality degradation in DASH streaming; (3) Potential improvement to TCP strategies for better delivery in DASH can be further explored.

==> Makefile <==
doc=main

all: $(doc).pdf

$(doc).pdf: *.tex sections/*.tex figures/*.eps mylib_short.bib
	latex $(doc).tex
	bibtex $(doc)
	latex $(doc).tex
	latex $(doc).tex
	dvipdfmx $(doc)
	
clean:
	rm -rf $(DOCUMENT).ps *.aux *.toc \
	*.blg *.bbl *.blg *.dvi *.mtc *.mtc? *.maf *.log *.out


==> sections/ack.tex <==
\section*{Acknowledgement}

The work is supported by National Significant Science and Technology Projects of China under Grant No. 2013ZX01039001-002-003, National Natural Science Foundation of China Project under Grant No.61170253, Promotion Project of Shenzhen Key Laboratory on Information Science and Technology 2012.


==> sections/discussion.tex <==
\section{Discussions} \label{sec:discuss}

Suppose that two DASH users A and B are watching videos, A's network speed is 180kbps and B's network speed is 470kbps, however there are only two video versions--100kbps and 500kbps provided. Both of them have to watch video of low quality. Users can acquire smooth and high quality video if they can modify the TCP competitiveness. User A also can watch the 100kbps video by reducing the TCP competitiveness while user B can get the 500kbps video by raising the TCP competitiveness.

Adjustment mentioned above  has a strong appeal to DASH users. If these adjustments can be embedded into the CDN server, then DASH video users can get the best video service allowed in their conditions. In order to achieve the above features, we first need to modify the current congestion control algorithm to improve transmission performance.

Based on the target for higher chunk transmission speed, we use an idea of using multiple virtual connections which can greatly promote the chunk  transmission efficiency. As shown in the Figure 9, download speed of our idea is much larger than the Cubic which Linux uses as congestion control method by default under conditions of RTT. We can learn that performance of multiple virtual connections is promoted 19.5\% compared with Cubic, which means DASH users can acquire a high quality video by using multiple virtual connections when service logs from the top ISP in China are considered. Except RTT, PLR also can reflect network status. Taking this fact into account, we have conducted experiments under PLR as shown in Figure 10.

Figure 10 depicts how two main chunk size transmission speeds change with the packet loss rate. Both chunk download speeds have shown a significant decline with the increase of packet loss rate. However, multiple virtual connections performs much better than the Cubic with 15.2\% promoted regardless of chunk size. 

Measurement results shown above mean we can get DASH video chunk transmission speed clearly promoted. Our future work is to modify the initial window size and competitiveness of multiple virtual connections according to the network status in the service side. Now we have implemented the portion of source code, which implies we can deploy it on the servers of Tencent DASH video in the near future and then we can acquire new useful logs to analyze and improve our algorithm.



